Symplectic isotopy of rational cuspidal sextics and septics

We classify rational cuspidal curves of degrees 6 and 7 in the complex projective plane, up to symplectic isotopy. The proof uses topological tools, pseudoholomorphic techniques, and birational transformations.

==> sections/auxiliary.tex <==
% !TEX root = ../septics.tex


